Contextual Slot Carryover for Disparate Schemas

In the slot-filling paradigm, where a user can refer back to slots in the context during a conversation, the goal of the contextual understanding system is to resolve the referring expressions to the appropriate slots in the context. In large-scale multi-domain systems, this presents two challenges - scaling to a very large and potentially unbounded set of slot values, and dealing with diverse schemas. We present a neural network architecture that addresses the slot value scalability challenge by reformulating the contextual interpretation as a decision to carryover a slot from a set of possible candidates. To deal with heterogenous schemas, we introduce a simple data-driven method for trans- forming the candidate slots. Our experiments show that our approach can scale to multiple domains and provides competitive results over a strong baseline.

==> related_work.tex <==
There is a rich body of work on coreference resolution for written text, which rely on clustering\cite{wellner2003towards, stoyanov2012easy, culotta2007first} or ranking mention pairs~\cite{durrett2013easy,wiseman2015learning}.  These have been extended to spoken dialog, by adding discourse specific features~\cite{rao2015dialogue, strube2003machine, Stent2010InteractionBD, liu2015deep}. However, most of these approaches follow a pipelined model of mention detection followed by coreference resolution; where linguistic features, syntax and discourse features are usually applied. In contrast, our proposed formulation does not rely on explicit linguistic features such as gender and type agreement, which are hard to acquire across languages. Furthermore, we can generalize the solution to sub-tasks such as zero pronouns naturally, as we don't have to explicitly identify the anaphoric mentions.

In addition there has been work on improving semantic frame error rate for current turn by leveraging context turns by encoding dialog states. ~\cite{bapna2017sequential} compare various approaches encoding context, ~\cite{chen2016end} describe a memory network architecture for knowledge carryover, adding semantic context from the frame ~\cite{yann2014zero}, using context features for domain classification ~\cite{xu2014contextual}. Our work differs from this body of literature, we keep the system for semantic frame prediction fixed and explore methods to explicitly add slots from previous turn. Previous work assumes existence of a dialog manager which can be used to keep track of entities to keep from previous turns.

A closely related approach is dialog state tracking~\cite{Williams2013TheDS, hori2016dialog, Henderson2013DeepNN}, where the system has to predict a set of slot-value pairs which matches the contents of the current segment. Usually, state trackers produce a distribution over all possible slot-value pairs; this does not scale for open-ended slot values (such as Date or Time), as well as slots whose values are constantly being updated (such as Songs, Movies). Our approach avoids this by reformulating the tracking problem as a carry-over action for the current turn. Recently, frame-tracking \cite{frametracking2017}, was introduced as an extension to state tracking, which also assigns slots to frames. A key difference here is that our formulation deals with the issue of disparate labels over a large-scale multi-domain system.



